To Observe or Not to Observe: Queuing Game Framework for Urban Parking

We model parking in urban centers as a set of parallel queues and overlay a game theoretic structure that allows us to compare the user-selected (Nash) equilibrium to the socially optimal equilibrium. We model arriving drivers as utility maximizers and consider the game in which observing the queue length is free as well as the game in which drivers must pay to observe the queue length. In both games, drivers must decide between balking and joining. We compare the Nash induced welfare to the socially optimal welfare. We find that gains to welfare do not require full information penetration---meaning, for social welfare to increase, not everyone needs to pay to observe. Through simulation, we explore a more complex scenario where drivers decide based the queueing game whether or not to enter a collection of queues over a network. We examine the occupancy-congestion relationship, an important relationship for determining the impact of parking resources on overall traffic congestion. Our simulated models use parameters informed by real-world data collected by the Seattle Department of Transportation.

==> back.tex <==
\label{sec:back}
%\todo{TO DO}

Dynamic pricing for traffic has received a lot of attention recently. For
example, see \cite{QianEtAl2014,
mackowski:2015aa,MartensBenensonLevy2010,QianRajagopal2014}. In these
works, occupancy is the main metric that is utilized for parking. A
desired occupancy rate is typically taken as an exogenous input to the
optimization problem and is 
indiscriminately targeted. While these techniques are not without merit, further
investigation into the fundamental relationship between parking usage and
congestion is needed.
Moreover, new metrics for parking utilization that factor in network topology
and socioeconomic factors need to be developed. 

Given a parallel queue model learned from the SDOT data,
we overlay a game-theoretic
structure that enables us to assess the effects of drivers' strategic behaviors.
Regardless of the level of granularity, the game is similar to the so-called \emph{supermarket
game} or \emph{tollbooth plaza problem} (see,
e.g.,~\cite{xu:2012aa,kim:2009aa}). As the name of the game suggests, it is used
to model the strategic interactions between users who are waiting to be served. 
When drivers choose a queue to enter based on 
user preference and available \emph{information}, which varies across the
population.

The \emph{value of information} and how it is
measured becomes very important in this game since it is a critical factor
in determining the equilibrium strategies of the agents. In addition, it is important
to understand how the value behaves as a function of the distribution of players
who do and do not have access to the information as it helps characterize
efficiency.
For example, we may consider the value of information to each player to be the
expected reduction in expected waiting time for parking due to an
increase in information~\cite{hassin:2011aa}.  
%A scenario that we can analyze is one in which

%Suppose a portion $p$ of the population purchases information at cost $C$
% while the remainder $1-p$ of the population
% opts-out. This may be the case if, say, there was an
%smartphone app that presents occupancy or another metric in near real-time for a
% cost $C$.
% %not  purchas the information. 
%If the value of information is
%characterized by the function $g(p)$, then we may determine the Nash equilibrium
%by finding $p$ that satisfies $g(p)=C$, i.e.~the cost of information should equal its
%value.  

%\tc{red}{inverse optimization}



 This framework lends itself naturally to the investigation of interesting
 strategic behaviors such as
\emph{jockeying} (changing between queues), \emph{balking} (choosing another
mode of transit), or
\emph{reneging} (selecting more expensive off-street
parking). While these more complex behaviors
have been studied for queuing games (see,
e.g.~\cite{hassin:1994aa,hassin:2003aa}), little is known about the case where
network constraints such as topology or capacity are
enforced. This means jockeying can only happen to neighboring queues and where
ability to jockey is directly a function of flow.
%and these
%behaviors have not been studied in a urban parking context. 
Moreover, much of the game-theoretic research for multiple
 parallel queues focuses on either $N=1,2$ or $N\rightarrow \infty$ queues and
 assumes Markovian characteristics; however, preliminary analysis of the SDOT data
 indicates that partitioning of the city into neighborhoods  modeled as parallel
 queues 
 results in a 
 more accurate model with a finite number of queues, larger than $2$, and general
 distribution for service times (i.e.~system of parallel M/G/$n$ queues). 



==> fig/supermarket.tex <==
\begin{tikzpicture}
  \node (head)
          {\includegraphics[scale=0.25]{fig/mindfls.png}};
          %\draw[bigg arrow, draw=sorange!45] (i)--(head);
          \node[right=0.75cm of head] (head1)
          {\includegraphics[scale=0.25]{fig/mindfls-empty.png}};
          \draw [NavyBlue!85!black,decorate,decoration={brace,amplitude=5pt, mirror},xshift=-4pt,yshift=0pt, very thick]
(-0.4,-0.75) -- (0.6,-0.75) node (q) [black,midway,xshift=-0.1cm] 
{}; 
\draw [NavyBlue!85!black,decorate,decoration={brace,amplitude=5pt, mirror},xshift=-4pt,yshift=0pt, very thick]
(1.85,-0.75) -- (2.85,-0.75) node (q2) [black,midway,xshift=-0.1cm] 
{}; 
\node[below=0.1cm of q,NavyBlue!85!black]   {\small $p$};
\node[below=0.1cm of q2,NavyBlue!85!black]   {\small $1-p$};


 \node[rbox99, fill=LimeGreen!25, draw=OliveGreen, below right=0.5cm and 4.75cm of q] (qu1)
          {queue 1};
           \node[rbox99, fill=LimeGreen!25, draw=OliveGreen, right=0.1cm of qu1]
           (qu2) {queue 2};
\node[right=0.1cm of qu2] (m1) {};
\fill[black] (m1) circle [radius=1.5pt]; 
\node[right=0.0cm of m1] (m2) {};
\fill[black] (m2) circle [radius=1.5pt]; 
\node[right=0.0cm of m2] (m3) {};
\fill[black] (m3) circle [radius=1.5pt]; 
\node[rbox99, fill=LimeGreen!25, draw=OliveGreen, right=0.1cm of m3]
           (qun) {queue $n$};
\node[above=0.0cm of qu1] (car1) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=-0.3cm of car1] (car2) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=-0.3cm of car2] (car3) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=-0.3cm of car3] (car4) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=0.0cm of qu2] (car31) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=-0.3cm of car31] (car41) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=0.0cm of qun] (car3n) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=-0.3cm of car3n] (car4n) {\includegraphics[scale=0.065]{fig/car.png}};
\node[above=-0.3cm of car4n] (car5n) {\includegraphics[scale=0.065]{fig/car.png}};

\end{tikzpicture}



==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2016cdc
# put the names of figure files here.  include the .eps
#figures = 
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
referencefile = 2016cdc

TEX = pdflatex

# support subdirectories
VPATH = Figs

# reruns latex if needed.  to get rid of this capability, delete the
# three lines after the rule.  Delete .bbl dependency if not using
# BibTeX references.
# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
$(latexfile).pdf : $(figures) $(latexfile).tex 
#$(latexfile).dvi : $(figures) $(latexfile).tex $(latexfile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
#%.eps : %.fig
#	fig2dev -L eps $< > $(dir $< )$@

#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf $(latexfile).ps $(latexfile).pdf

#pdf : $(latexfile).pdf

#$(latexfile).ps : $(latexfile).dvi
#	dvips $(latexfile)

#ps : $(latexfile).ps 

# make can't know all the sourcefiles.  some file may not have
# sourcefiles, e.g. eps's taken from other documents. 
#$(latexfile).tar.gz : $(figures) $(latexfile).tex $(referencefile).bib
#	tar -czvf $(latexfile).tar.gz $^

#tarball: $(latexfile).tar.gz

cpall:
	make; skim $(latexfile).pdf

clean:
	rm $(latexfile).dvi $(latexfile).log $(latexfile).ps $(latexfile).pdf

fixpdf:
	gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=fixed.pdf $(latexfile).pdf

mpdf:
	pdflatex $(latexfile).tex; skim $(latexfile).pdf

bibit: 
	bibtex $(latexfile); mpdf



